Java Decompiler Diversity and its Application to Meta-decompilation

During compilation from Java source code to bytecode, some information is irreversibly lost. In other words, compilation and decompilation of Java code is not symmetric. Consequently, decompilation, which aims at producing source code from bytecode, relies on strategies to reconstruct the information that has been lost. Different Java decompilers use distinct strategies to achieve proper decompilation. In this work, we hypothesize that the diverse ways in which bytecode can be decompiled has a direct impact on the quality of the source code produced by decompilers. In this paper, we assess the strategies of eight Java decompilers with respect to three quality indicators: syntactic correctness, syntactic distortion and semantic equivalence modulo inputs. Our results show that no single modern decompiler is able to correctly handle the variety of bytecode structures coming from real-world programs. The highest ranking decompiler in this study produces syntactically correct, and semantically equivalent code output for 84%, respectively 78%, of the classes in our dataset. Our results demonstrate that each decompiler correctly handles a different set of bytecode classes. We propose a new decompiler called Arlecchino that leverages the diversity of existing decompilers. To do so, we merge partial decompilation into a new one based on compilation errors. Arlecchino handles 37.6% of bytecode classes that were previously handled by no decompiler. We publish the sources of this new bytecode decompiler.

==> listings/CFR-MaxHistory.tex <==
\textbf{}\begin{lstlisting}[style=Java, float, floatplacement=H, caption={Excerpt of org.junit.experimental.max.MaxHistory decompiled with \cfr .}, label={lst:maxhistory-cfr},belowskip=-6\baselineskip]
public class MaxHistory implements Serializable {
    [...]
    public RunListener listener() {
        return new RememberingListener();
    }

    public Comparator<Description> testComparator() {
        return new TestComparator();
    }
    
    private static MaxHistory readHistory(File storedResults) throws CouldNotReadCoreException {
        try {
            FileInputStream file = new FileInputStream(storedResults);
            try {
                MaxHistory maxHistory;
                ObjectInputStream stream = new ObjectInputStream(file);
                try {
                    maxHistory = (MaxHistory)stream.readObject();
                }
                catch (Throwable throwable) {
                    stream.close();
                    throw throwable;//Compilation error
                }
                stream.close();
                return maxHistory;
            }
            finally {
                file.close();
            }
        }
        catch (Exception e) {
            throw new CouldNotReadCoreException(e);
        }
    }
}
\end{lstlisting}

==> listings/Foo-Fernflower.tex <==
\begin{lstlisting}[style = Java, float, floatplacement=H, caption={Foo decompiled with \fernflower.}, label={lst:foo-fernflower},belowskip=-6\baselineskip]
public class Foo {
  public int foo(int i, int j) {
   while(true) {
     try {
      while(i < j) i = j++ / i;
      ~return j;~
     } catch (RuntimeException var4) {
      i = 10;
     }
   }
  }
}
\end{lstlisting}

==> listings/MutableObject-Fernflower.tex <==
\begin{lstlisting}[style=Java, float, floatplacement=H, caption={Excerpt of differences in MutableObject original and decompiled with \fernflower sources.}, label={lst:mutable-object-fernflower},belowskip=-6\baselineskip]
    public static int toIntValue(final char ch) {...}
	
    public static int toIntValue(final Character ch) {
        Validate.isTrue(ch != null, "The character must not be null");
        `return toIntValue(ch.charValue());`
        £return toIntValue(ch);£
    }
\end{lstlisting}

==> listings/Procyon-MaxHistory.tex <==
\textbf{}\begin{lstlisting}[style=Java, float, floatplacement=H, caption={Excerpt of org.junit.experimental.max.MaxHistory decompiled with \procyon .}, label={lst:maxhistory-procyon},belowskip=-6\baselineskip]
public class MaxHistory implements Serializable {
    [...]
    public RunListener listener() {
        //Compilation error
        return new RememberingListener((RememberingListener)null);
    }
    
    public Comparator<Description> testComparator() {
        //Compilation error
        return new TestComparator((TestComparator)null);
    }
    
    private static MaxHistory readHistory(final File storedResults) throws CouldNotReadCoreException {
        try {
            final FileInputStream file = new FileInputStream(storedResults);
            try {
                final ObjectInputStream stream = new ObjectInputStream(file);
                try {
                    return (MaxHistory)stream.readObject();
                }
                finally {
                    stream.close();
                }
            }
            finally {
                file.close();
            }
        }
        catch (Exception e) {
            throw new CouldNotReadCoreException(e);
        }
    }
}
\end{lstlisting}

==> listings/bukkit-jadx-1-decompiled.tex <==
\begin{lstlisting}[style=Java, float, floatplacement=H, caption={Exerpt of org/bukkit/Bukkit.java decompiled.}, label={lst:bukkit-decompiled},belowskip=-6\baselineskip] 
public final class Bukkit {
    £private static Server server;£
	[...]
    public static void setServer(Server server) {
        if (server != null) {
            throw new UnsupportedOperationException(
            "Cannot redefine singleton Server");
        }
        ~server = server;~
        [...]
    }
\end{lstlisting}

==> tables/diff.tex <==
\begin{table}[ht!]
\centering
\caption{Bytecode difference ratios of recompilable and pass test classes for each decompiler}
\footnotesize
\begin{tabular}{lcccc}
			\hline
			\textbf{Decompiler}  & \textbf{Diff $==$ 0} & \textbf{Diff $\neq$ 0} & \textbf{Ratio} & \textbf{Ratio (Int)} \\
			\hline
    		\cfr & 1114 & 599 & 0.65 & 0.84\\
    		\fernflower & 582 & 853 & 0.41 & 0.59 \\
    		\krakatau  &  187 & 537 &  0.26 & 0.43\\
    		\procyon  & 1278 & 579 & 0.69 & 0.91\\
    		\dava & 173 & 589 & 0.23 & 0.38\\
    		\jd & 1142 & 233 & 0.83 & 0.87\\
    		\jode & 596 & 539 & 0.53 & 0.68\\
    		\jadx & 573 & 835 & 0.41 & 0.59\\
            \hline
		\end{tabular}
	\label{tab:bytecode-diff}
\end{table}



==> utils/util.tex <==
\usepackage{soul}
\usepackage{tikz}

\usetikzlibrary{calc}
\usetikzlibrary{decorations.pathmorphing}

\makeatletter

\newcommand{\defhighlighter}[3][]{%
  \tikzset{every highlighter/.style={color=#2, fill opacity=#3, #1}}%
}

\defhighlighter{yellow}{.5}

\newcommand{\highlight@DoHighlight}{
  \fill [ decoration = {random steps, amplitude=1pt, segment length=15pt}
        , outer sep = -15pt, inner sep = 0pt, decorate
        , every highlighter, this highlighter ]
        ($(begin highlight)+(0,8pt)$) rectangle ($(end highlight)+(0,-3pt)$) ;
}

\newcommand{\highlight@BeginHighlight}{
  \coordinate (begin highlight) at (0,0) ;
}

\newcommand{\highlight@EndHighlight}{
  \coordinate (end highlight) at (0,0) ;
}

\newdimen\highlight@previous
\newdimen\highlight@current

\DeclareRobustCommand*\highlight[1][]{%
  \tikzset{this highlighter/.style={#1}}%
  \SOUL@setup
  %
  \def\SOUL@preamble{%
    \begin{tikzpicture}[overlay, remember picture]
      \highlight@BeginHighlight
      \highlight@EndHighlight
    \end{tikzpicture}%
  }%
  %
  \def\SOUL@postamble{%
    \begin{tikzpicture}[overlay, remember picture]
      \highlight@EndHighlight
      \highlight@DoHighlight
    \end{tikzpicture}%
  }%
  %
  \def\SOUL@everyhyphen{%
    \discretionary{%
      \SOUL@setkern\SOUL@hyphkern
      \SOUL@sethyphenchar
      \tikz[overlay, remember picture] \highlight@EndHighlight ;%
    }{%
    }{%
      \SOUL@setkern\SOUL@charkern
    }%
  }%
  %
  \def\SOUL@everyexhyphen##1{%
    \SOUL@setkern\SOUL@hyphkern
    \hbox{##1}%
    \discretionary{%
      \tikz[overlay, remember picture] \highlight@EndHighlight ;%
    }{%
    }{%
      \SOUL@setkern\SOUL@charkern
    }%
  }%
  %
  \def\SOUL@everysyllable{%
    \begin{tikzpicture}[overlay, remember picture]
      \path let \p0 = (begin highlight), \p1 = (0,0) in \pgfextra
        \global\highlight@previous=\y0
        \global\highlight@current =\y1
      \endpgfextra (0,0) ;
      \ifdim\highlight@current < \highlight@previous
        \highlight@DoHighlight
        \highlight@BeginHighlight
      \fi
    \end{tikzpicture}%
    \the\SOUL@syllable
    \tikz[overlay, remember picture] \highlight@EndHighlight ;%
  }%
  \SOUL@
}

\makeatother

% Common abbrev. are set as commands to ensure proper spacing after the dot
\newcommand{\ie}{i.e.\@\xspace}
\newcommand{\aka}{a.k.a.\@\xspace}
\newcommand{\Aka}{A.k.a.\@\xspace}
\newcommand{\Ie}{I.e.\@\xspace}
\newcommand{\cf}{cf.\@\xspace}
\newcommand{\Cf}{Cf.\@\xspace}
\newcommand{\eg}{e.g.\@\xspace}
\newcommand{\Eg}{E.g.\@\xspace}
\newcommand{\etal}{et al.\@\xspace}
\newcommand{\etc}{etc.\@\xspace}
\newcommand{\wrt}{w.r.t.\@\xspace}
\newcommand{\Wrt}{W.r.t.\@\xspace}
\newcommand{\mc}{Maven Central\@\xspace}
\newcommand{\semi}{semantic equivalence modulo inputs\@\xspace}
\newcommand{\latests}{\text{\texttt{LATESTS}\@\xspace}}
\newcommand{\pas}{\text{\texttt{P}\@\xspace}}
\newcommand{\act}{\text{\texttt{A}\@\xspace}}
\newcommand{\latest}{\text{$latest$\@\xspace}}
\newcommand{\notlatests}{\overline{\latests}}%% NOTE, it should be used in Math mode!

% List of considered decompilers
\newcommand{\krakatau}{\textsf{Krakatau}\@\xspace}
\newcommand{\jode}{\textsf{Jode}\@\xspace}
\newcommand{\cfr}{\textsf{CFR}\@\xspace}
\newcommand{\fernflower}{\textsf{Fernflower}\@\xspace}
\newcommand{\procyon}{\textsf{Procyon}\@\xspace}
%\newcommand{\jd}{\textsf{JD-GUI}\@\xspace}
\newcommand{\jd}{\textsf{JD-Core}\@\xspace}
\newcommand{\jadx}{\textsf{JADX}\@\xspace}
\newcommand{\dava}{\textsf{Dava}\@\xspace}
\newcommand{\meta}{\textsf{Multi-DC}\@\xspace}

%\newcommand{\metadc}{\textsf{MetaDecompiler}\@\xspace}
\newcommand{\metadc}{\textsf{Arlecchino}\@\xspace}


\newcommand{\javac}{\textit{javac}\@\xspace}
\newcommand{\ecj}{\textit{ecj}\@\xspace}

\newcommand{\mdg}{MDG\@\xspace}
\newcommand{\mdgl}{$\text{MDG}_L$\@\xspace}
\newcommand{\start}{\texttt{START}\@\xspace}
\newcommand{\snapshot}{\texttt{SNAPSHOT}\@\xspace}
\newcommand{\isPassive}{isPsv}
\newcommand{\orderV}{\displaystyle {<}_{v}}
\newcommand{\orderT}{\displaystyle {<}_{t}}
\newcommand{\lib}{\texttt{LIBS}\@\xspace}

% comment commands for co-authors
\newcommand{\nicolas}[1]{\mynote{Nicolas}{#1}}
\newcommand{\cesar}[1]{\mynote{Cesar}{#1}}
\newcommand{\martin}[1]{\mynote{Martin}{#1}}
\newcommand{\benoit}[1]{\mynote{Benoit}{#1}}
% \renewcommand{\todo}[1]{\mynote{todo}{#1}}

%\newcommand{\nbartifacts}{$1,487,956$\@\xspace}
%\newcommand{\nblibraries}{$73,653$\@\xspace}
\newcommand\highlightred[1]{\colorbox{red!17}{#1}}



\newcommand{\mstore}{Fragment Store\xspace}
\newcommand{\store}{fragment store\xspace}

\newcommand{\modified}[1]{{\color{blue}#1}} 
%\newcommand{\modified}[1]{#1} 
%\newcommand\textvtt[1]{{\normalfont\fontfamily{cmvtt}\selectfont #1}}
